Hybrid Projection Methods with Recycling for Inverse Problems

Iterative hybrid projection methods have proven to be very effective for solving large linear inverse problems due to their inherent regularizing properties as well as the added flexibility to select regularization parameters adaptively. In this work, we develop Golub-Kahan-based hybrid projection methods that can exploit compression and recycling techniques in order to solve a broad class of inverse problems where memory requirements or high computational cost may otherwise be prohibitive. For problems that have many unknown parameters and require many iterations, hybrid projection methods with recycling can be used to compress and recycle the solution basis vectors to reduce the number of solution basis vectors that must be stored, while obtaining a solution accuracy that is comparable to that of standard methods. If reorthogonalization is required, this may also reduce computational cost substantially. In other scenarios, such as streaming data problems or inverse problems with multiple datasets, hybrid projection methods with recycling can be used to efficiently integrate previously computed information for faster and better reconstruction. Additional benefits of the proposed methods are that various subspace selection and compression techniques can be incorporated, standard techniques for automatic regularization parameter selection can be used, and the methods can be applied multiple times in an iterative fashion. Theoretical results show that, under reasonable conditions, regularized solutions for our proposed recycling hybrid method remain close to regularized solutions for standard hybrid methods and reveal important connections among the resulting projection matrices. Numerical examples from image processing show the potential benefits of combining recycling with hybrid projection methods.

==> in_storage.tex <==



%% Theoreom
\begin{theorem}
\label{theinter1}
Let $\bfV_{m+\ell}$, $\bfU_{m+\ell+1}$, and $\bfB_{m+\ell}$ be the matrices computed after $m+\ell$ iterations of GKB.
Assume that $\bfx^{(0)}$ is an arbitrary regularized solution computed from $\calR(\bfV_{m})$ and $\bfW_{k-1}$ is obtained using TSVD compression of $\bfV_m$.
% Then with $\bfW_{k} = [\bfW_{k-1} \quad \bfx^{(1)}]$,
After $\ell$ iterations of recycling GKB, we have $\wt{\bfU}_{\ell+1} = [\wt{\bfu}_{1}, \dots, \wt{\bfu}_{\ell+1}]$, $\wt{\bfV}_{\ell} = [\wt{\bfv}_{1}, \dots, \wt{\bfv}_{\ell}]$, and $\widehat{\bfB}_{k,\ell}.$  Then there exist orthogonal matrices $\begin{bmatrix} \bfT & \bfT_c\end{bmatrix}$ and $\begin{bmatrix} \bfZ & \bfZ_c\end{bmatrix}$ such that
% Let $\bfx_m$ be an arbitrary regularized solution computed from $\calR(\bfV_{m})$. $\bfW_{k} = [\bfW_{k-1} \quad \bfx^{(1)}]$, where $\bfx^{(1)} = (\bfI - \bfW_{k-1}\bfW_{k-1}\t)\bfx_{m}$. Then
\begin{equation}
\label{thm:bbhat}
\begin{bmatrix}\bfT^{\top} \\ \bfT^{\top}_{c}\end{bmatrix} \bfB_{m+\ell} \begin{bmatrix}\bfZ & \bfZ_{c}\end{bmatrix}  = \begin{bmatrix}\widehat{\bfB}_{k,\ell} & \bfT^{\top}\bfB_{m+\ell}\bfZ_c \\ \bfzero & \bfT^{\top}_{c}\bfB_{m+\ell}\bfZ_{c}\end{bmatrix}.
\end{equation}
Furthermore, for $j = 1, \dots, k+\ell$
\begin{align}
\label{eq4}
\sigma_{m-k+j}(\bfB_{m+\ell}) \le \sigma_{j}(\widehat{\bfB}_{k,\ell}) \le \sigma_{j}(\bfB_{m+\ell})
\end{align}
where $\sigma_{j}(\cdot)$ denotes the $j-$th singular value of a matrix.

\begin{proof}
Let the TSVD of $\bfB_m$ be
\begin{equation}
\label{TSVD}
\bfB_m \approx {\bf\Psi}_{k-1}{\bf\Sigma}_{k-1}{\bf\Phi}_{k-1}^{\top}
\end{equation}
and SVD of $\bfB_{m}$ be
\begin{equation}
\label{SVD}
\bfB_m = {\bf\Psi}_{m+1}{\bf\Sigma}_{m}{\bf\Phi}_{m}^{\top},
\end{equation}
where ${\bf\Psi}_{m+1} \in \mathbb{R}^{(m+1)\times(m+1)}$, ${\bf\Phi}_{m} \in \mathbb{R}^{m \times m}$ are unitary matrices, ${\bf\Psi}_{k-1} \in \mathbb{R}^{(m+1)\times(k-1)}$, ${\bf\Phi}_{k-1} \in \mathbb{R}^{m \times (k-1)}$ have orthonormal columns and
\begin{equation}
{\bf\Sigma}_{m} = \begin{bmatrix}\sigma_1 & & \\ & \ddots &\\ & & \sigma_m \\& & 0 \end{bmatrix} \in \mathbb{R}^{(m+1) \times m}, \qquad {\bf\Sigma}_{k-1} = \begin{bmatrix}\sigma_1 & & \\ & \ddots &\\ & & \sigma_{k-1} \end{bmatrix} \in \mathbb{R}^{(k-1) \times (k-1)}
\end{equation}
are diagonal matrices with nonincreasing singular values. Based on the relationship between TSVD and SVD,
\begin{align}
\label{relationship1}
{\bf\Psi}_{m+1} &= \begin{bmatrix}{\bf\Psi}_{k-1} & {\bf\Psi}_{c}\end{bmatrix}\\
\label{relationship2}
{\bf\Phi}_{m} &= \begin{bmatrix}{\bf\Phi}_{k-1} & {\bf\Phi}_{c}\end{bmatrix}\\
\label{relationship3}
{\bfSigma}_{m} &= \begin{bmatrix}{\bfSigma}_{k-1} & \bf0\\ \bf0 & {\bfSigma}_{c}  \end{bmatrix},
\end{align}
where ${\bf\Psi}_{c} \in \mathbb{R}^{(m+1) \times (m+2-k)} \perp {\bf\Psi}_{k-1}$, ${\bf\Phi}_{c} \in \mathbb{R}^{m \times (m+1-k)} \perp {\bf\Phi}_{k-1}$, and ${\bfSigma}_{c}  = \begin{bmatrix}\sigma_k & & \\ & \ddots &\\ & & \sigma_m \\& & 0 \end{bmatrix} \in \mathbb{R}^{(m-k+2)\times(m-k+1)}$.
By (\ref{TSVDW}),
\begin{align*}
\bfA\bfW_k &= \bfA\bfV_{m}{\bf\Phi}_{k-1} \\
              &= \bfU_{m+1}\bfB_{m}{\bf\Phi}_{k-1} \\
              & = \bfU_{m+1}{\bf\Psi}_{m+1}\bfSigma_{m}{\bf\Phi}_{m}\t{\bf\Phi}_{k-1}\\
              & = \bfU_{m+1}{\bf\Psi}_{m+1}\bfSigma_{m}{\begin{bmatrix}\bfI_{(k-1)\times(k-1)}\\\bfO_{(m-k+1)\times(k-1)}\end{bmatrix}}\\
              & = \bfU_{m+1}{\bf\Psi}_{k-1}\bfSigma_{k-1}.
\end{align*}
Let $\wt{\bfY} = \bfU_{m+1}{\bf\Psi}_{k-1}$ and $\bfA\bfx^{(1)} = \wt{\bfY}\wt{\bfY}\t\bfA\bfx^{(1)} + \bfy_{k}r_{kk}$. Since $\bfA\bfW_{k}$ is full rank, $\bfY_{k}$ and $\bfR_{k}$ in QR factorization (\ref{AWYR}) can be written uniquely and explicitly as
\begin{equation*}
\bfY_{k} = \begin{bmatrix}\wt{\bfY} & \bfy_{k}\end{bmatrix} \quad \bfR_{k} = \begin{bmatrix} {\bf\Sigma}_{k-1} & \wt{\bfY}\t\bfA\bfx^{(1)} \\ \bfO_{1\times (k-1)} & r_{kk}\end{bmatrix}.
\end{equation*}
According to Lemma \ref{lem3},
\begin{align}
\label{eq:wvproof}
\begin{bmatrix}\bfW_{k}& \wt{\bfV}_{\ell}\end{bmatrix} &=  \begin{bmatrix}\bfV_{m}{\bf\Phi}_{k-1}& \bfx^{(1)}&\wt{\bfV}_{\ell}\end{bmatrix} = \bfV_{m+\ell}\begin{bmatrix} {\bf\Phi}_{k-1} & \xi & \wt{\bfZ}_{1}  \\ \bfO_{\ell\times (k-1)} & \bfO_{\ell \times 1} & \wt{\bfZ}_{2} \end{bmatrix} = \bfV_{m+\ell}\bfZ, \\
\label{eq:yuproof}
\begin{bmatrix} \bfY_{k} & \wt{\bfU}_{\ell+1} \end{bmatrix} &= \bfU_{m+\ell+1}\begin{bmatrix} {\bf\Psi}_{k-1} & \eta & \wt{\bfT}_{1}  \\ \bfO_{\ell \times (k-1)} & \bfO_{\ell \times 1} & \wt{\bfT}_{2} \end{bmatrix} = \bfU_{m+\ell+1}\bfT,
\end{align}
where $\bfZ = \begin{bmatrix} {\bf\Phi}_{k-1} & \xi & \wt{\bfZ}_{1}  \\ \bfO_{\ell\times (k-1)} & \bfO_{\ell \times 1} & \wt{\bfZ}_{2} \end{bmatrix} \in \mathbb{R}^{(m+\ell)\times(k+\ell)}$ and $\bfT = \begin{bmatrix} {\bf\Psi}_{k-1} & \eta & \wt{\bfT}_{1}  \\ \bfO_{\ell \times (k-1)} & \bfO_{\ell \times 1} & \wt{\bfT}_{2} \end{bmatrix}\in \mathbb{R}^{(m+\ell+1)\times(k+\ell)}$ have orthonormal columns. By (\ref{eq:new_gkb}) and (\ref{eq:yuproof}),
\begin{align*}
\bfU_{m+\ell+1}\bfB_{m+\ell} &= \bfA\bfV_{m+\ell} \\
\bfT\t\bfB_{m+\ell}\bfZ &= \bfT\t\bfU\t_{m+\ell+1}\bfA\bfV_{m+\ell}\bfZ\\
&=\bfT\t\bfU^{\top}_{m+\ell+1}\bfA\begin{bmatrix}\bfW_{k}& \wt{\bfV}_{\ell}\end{bmatrix}\\
&= \bfT\t\bfU\t_{m+\ell+1}\begin{bmatrix} \bfY_{k} & \wt{\bfU}_{\ell+1} \end{bmatrix}\widehat{\bfB}_{k,\ell}\\
&= \bfT^{\top}\bfU^{\top}_{m+\ell+1}\bfU_{m+\ell+1}\bfT \widehat{\bfB}_{k,\ell}\\
&= \widehat{\bfB}_{k,\ell}.
\end{align*}
Let $\bfT_{c}$ and $\bfZ_{c}$ orthogonal complements of $\bfT$ and $\bfZ$ respectively. Then
\begin{equation}
\label{eq:bbhat}
\begin{bmatrix}\bfT^{\top} \\ \bfT^{\top}_{c}\end{bmatrix} \bfB_{m+\ell} \begin{bmatrix}\bfZ & \bfZ_{c}\end{bmatrix}  = \begin{bmatrix}\widehat{\bfB}_{k,\ell} & \bfT^{\top}\bfB_{m+\ell}\bfZ_{c} \\ \bfT^{\top}_{c}\bfB_{m+\ell}\bfZ & \bfT^{\top}_{c}\bfB_{m+\ell}\bfZ_{c}\end{bmatrix}
\end{equation}.
By (\ref{eq:new_gkb}), (\ref{eq:wvproof}) and (\ref{eq:yuproof}),
\begin{align}
\label{eq:new_gkb1}
\bfA\bfV_{m+\ell}\bfZ &= \bfU_{m+\ell+1}\bfT \widehat{\bfB}_{k,\ell} \\
\bfU_{m+\ell+1}\bfB_{m+\ell}\bfZ &= \bfU_{m+\ell+1}\bfT \widehat{\bfB}_{k,\ell}\\
\bfB_{m+\ell}\bfZ &= \bfT \widehat{\bfB}_{k,\ell} \\
\bfT_{c}^{\top}\bfB_{m+\ell}\bfZ &= \bfT_{c}^{\top}\bfT \widehat{\bfB}_{k,\ell}\\
&= \bfO_{(m+1-k) \times (k+\ell)},
\end{align}
since $\bfT_c$ is orthogonal to $\bfT$. Then (\ref{thm:bbhat}) is proved.
%proves (\ref{eq4}).\\
\end{proof}
\end{theorem}

\begin{theorem}
\label{thm_frobienius_norm}
Let $\sigma_{k}$ is the $k-$th largest singular value of $\bfB_{m}$ and
\begin{equation*}
\overline{\mxB}_{\ell} =\begin{bmatrix}
		\beta_{m+2} & \alpha_{m+2}& & \\
		 & \ddots& \ddots & \\
		 & & \beta_{m+\ell} & \alpha_{m+\ell} \\
		 & & & \beta_{m+\ell+1}  \\
	\end{bmatrix}\in \bbR^{\ell \times \ell}.
\end{equation*}
Then
\begin{equation}
\label{eq:frobupbd}
\norm[F]{\bfB_{m+\ell}} - \norm[F]{\widehat{\bfB}_{k,\ell}} \le \max\{\sigma_k, \norm[F]{\overline{\mxB}_{\ell}}\}(m-k) + |\alpha_{m+1}|.
\end{equation}
%where $C_{m,k,\ell}$ is a constant with respect to $m,k,\ell$.

\begin{proof}
Let
\begin{equation*}
\bfB_{m+\ell} = \begin{bmatrix}\bfB_{m} & \begin{bmatrix}\bfO_{m\times \ell} \\ \alpha_{m+1}\bfe_1\t \end{bmatrix} \\\\ \bfO_{\ell \times m} &  \overline{\bfB}_{\ell}\end{bmatrix}.
\end{equation*}
Define $\bfT_{c} = \begin{bmatrix}\wt{\bfT}_3 \\ \wt{\bfT}_4\end{bmatrix}$ and $\bfZ_{c} = \begin{bmatrix}\wt{\bfZ}_3 \\ \wt{\bfZ}_4\end{bmatrix}$, where $\wt{\bfT}_3 \in \mathbb{R}^{(m+1)\times(m-k+1)}$, $\wt{\bfT}_4 \in \mathbb{R}^{\ell\times(m-k+1)}$, $\wt{\bfZ}_3 \in \mathbb{R}^{m\times(m-k)}$ and $\wt{\bfZ}_4 \in \mathbb{R}^{\ell\times(m-k)}$.  Since $\bfT_{c} \perp \bfT$ and $\bfZ_{c} \perp \bfZ$,
\begin{align}
\label{eq:perp1}
\wt{\bfT}_3\t{\bf\Psi}_{k-1} &= \bfO_{(m-k+1)\times(k-1)} \\
\label{eq:perp2}
{\bf\Phi}_{k-1}\t\wt{\bfZ}_3 &= \bfO_{(k-1)\times(m-k)}
\end{align}
According to (\ref{thm:bbhat})in theorem \ref{theinter1},
\begin{align}
\label{frobdiff}
\norm[F]{\bfB_{m+\ell}} - \norm[F]{\widehat{\bfB}_{k,\ell}} &= \norm[F]{\bfT^{\top}\bfB_{m+\ell}\bfZ_c} + \norm[F]{\bfT^{\top}_c\bfB_{m+\ell}\bfZ_c} \\
& = \norm[F]{\begin{bmatrix}\bfT & \bfT_c\end{bmatrix}^{\top}\bfB_{m+\ell}\bfZ_c}\\
& = \norm[F]{\bfB_{m+\ell}\bfZ_c}\\
\label{diffright}
& = \norm[F]{\begin{bmatrix}\bfB_m\widetilde{\bfZ}_3 + \alpha_{m+1}\bfE_{m+1,1}\widetilde{\bfZ}_4 \\ \overline{\mxB}_{\ell}\widetilde{\bfZ}_4\end{bmatrix}},
\end{align}

%Thus,
%\begin{align}
%\bfT\t_{c}\bfB_{m+\ell}\bfZ &= \begin{bmatrix}\wt{\bfT}_3\t & \wt{\bfT}_4\t \end{bmatrix}\begin{bmatrix}\bfB_{m} & \begin{bmatrix}\bfO_{m\times \ell} \\ \alpha_{m+1}\bfe_1\t \end{bmatrix} \\\\ \bfO_{\ell \times m} & \overline{\bfB}_{\ell}\end{bmatrix}\begin{bmatrix} {\bf\Phi}_{k-1} & \xi & \wt{\bfZ}_{1}  \\ \bfO_{\ell\times (k-1)} & \bfO_{\ell \times 1} & \wt{\bfZ}_{2} \end{bmatrix} \\
%\label{eq:def1}
%&= \begin{bmatrix}\wt{\bfT}_3\t \bfB_{m}{\bf\Phi}_{k-1} & \wt{\bfT}_3\t \bfB_{m} \xi &  \wt{\bfT}_3\t \bfB_{m} \wt{\bfZ}_{1} + \wt{\bfT}_4\t  \overline{\bfB}_{\ell} \wt{\bfZ}_{2} + \alpha_{m+1}\wt{\bfT}_3\t \bfE_{m+1,1}\wt{\bfZ}_2\end{bmatrix},
%\end{align}
where $\bfE_{m+1,1} = \begin{bmatrix}\bfO_{m \times \ell} \\ \begin{bmatrix}1 & \bfO_{1 \times (\ell-1)}\end{bmatrix}\end{bmatrix} \in \mathbb{R}^{(m+1)\times \ell}$.
%Since $\bf\Psi_{k-1}$ Let
%${\bf\Phi}_{m} = \begin{bmatrix}{\bf\Phi}_{k-1} & {\bf\Phi}_{c}\end{bmatrix}$, ${\bf\Psi}_{m+1} = \begin{bmatrix}{\bf\Psi}_{k-1} & {\bf\Psi}_{c}\end{bmatrix}$ and ${\bf\Sigma}_{m} = \begin{bmatrix}{\bf\Sigma}_{k-1} &  \\ &{\bf\Sigma}_{c}\end{bmatrix}$, where
%\begin{equation*}
%{\bf\Sigma}_{c} =\begin{bmatrix}
%		\sigma_{k} & & & \\
%		   & \sigma_{k+1}& & \\
%		 & & \ddots & \\
%		 & & & \sigma_{m} \\
%		 & & & 0  \\
%	\end{bmatrix}\in \mathbb{R}^{(m-k+2) \times (m-k+1)}.
%\end{equation*}
%Based on (\ref{eq:perp1}),
%\begin{align}
%\wt{\bfT}_3\t \bfB_{m}  &= \wt{\bfT}_3\t {\bf\Psi}_{m+1} \Sigma_{m} {\bf\Phi}_{m}\t\\
%                          &= \wt{\bfT}_3\t \begin{bmatrix}{\bf\Psi}_{k} & {\bf\Psi}_{c}\end{bmatrix} \begin{bmatrix}{\bf\Sigma}_{k-1} &  \\ &{\bf\Sigma}_{c}\end{bmatrix} \begin{bmatrix}{\bf\Phi}_{k-1}\t \\\\ {\bf\Phi}_{c}\t\end{bmatrix} \\
%                          &= \begin{bmatrix}\bfO_{(m-k+1)\times(k-1)} & \wt{\bfT}_3\t{\bf\Psi}_{c} \end{bmatrix}\begin{bmatrix}{\bf\Sigma}_{k-1} &  \\ &{\bf\Sigma}_{c}\end{bmatrix} \begin{bmatrix}{\bf\Phi}_{k-1}\t \\\\ {\bf\Phi}_{c}\t\end{bmatrix} \\
%\label{eq:tb}
%                          &= \wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t.
%\end{align}
%Then
%\begin{align*}
%\wt{\bfT}_3\t \bfB_{m}{\bf\Phi}_{k-1} &= \wt{\bfT}_3\t {\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t{\bf\Phi}_{k-1}\\
%                                     &=\bfO_{(m-k+1)\times(k-1)}.
%\end{align*}
%Plug (\ref{eq:tb}) in (\ref{eq:def1}) and then
%\begin{equation*}
%\bfT^{\top}_{c}\bfB_{m+\ell}\bfZ = \begin{bmatrix}\bfO_{(m-k+1)\times(k-1)} & \wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t \xi &  \wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t\wt{\bfZ}_{1} + \wt{\bfT}^{\top}_4  \overline{\bfB}_{\ell} \wt{\bfZ}_{2} + \alpha_{m+1}\wt{\bfT}_3\t \bfE_{m+1,1}\wt{\bfZ}_2\end{bmatrix},
%\end{equation*}
%and
%\begin{equation*}
%\norm[F]{\bfT^{\top}_{c}\bfB_{m+\ell}\bfZ}^2 = \norm[F]{\wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t \xi}^2 + \norm[F]{\wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t\wt{\bfZ}_{1} + \wt{\bfT}^{\top}_4  \overline{\bfB}_{\ell} \wt{\bfZ}_{2} + \alpha_{m+1}\wt{\bfT}_3\t \bfE_{m+1,1}\wt{\bfZ}_2}^2.
%\end{equation*}
Since $\begin{bmatrix}\wt{\bfZ}_{3}\\ \wt{\bfZ}_{4}\end{bmatrix}$ are matrix with orthonormal columns,
\begin{align}
\label{ineq_1}
\norm[F]{\wt{\bfZ}_3}^2 + \norm[F]{\wt{\bfZ}_4}^2 &= \norm[F]{\bfZ_{c}}^2 = m-k\\
%\label{ineq_2}
%\norm[F]{\wt{\bfZ}_{1}}^2 + \norm[F]{\wt{\bfZ}_{2}}^2 &= \norm[F]{\begin{bmatrix}\wt{\bfZ}_{1}\\ \wt{\bfZ}_{2}\end{bmatrix}}^2 = \ell.
\end{align}
%In addition, ${\bf\Psi}_{c}, {\bf\Phi}_{c}, \xi$ are matrix(vector) with orthonormal column(s). Thus,
%\begin{align*}
%\norm[F]{\wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t \xi} &\le \sigma_{k}
%%\norm[F]{\wt{\bfT}^{T}_3\bfU_{Bc}\bfV^{T}_{Bc} \xi}\\
%%&\le \sigma_{k}\norm[F]{\wt{\bfT}^{T}_3}\norm[F]{\bfU_{Bc}}\norm[F]{\bfV^{T}_{Bc}}\norm[F]{\xi}\\
%%&\le \mathcal{C}^{1}_{m,k,\ell}\sigma_{k}.
%\end{align*}
%Similarly,
%\begin{align*}
%\norm[F]{\wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t\wt{\bfZ}_{1} + \wt{\bfT}_4\t  \overline{\bfB}_{\ell} \wt{\bfZ}_{2} + \alpha_{m+1}\wt{\bfT}_3\t \bfE_{m+1,1}\wt{\bfZ}_2} &\le \norm[F]{\wt{\bfT}_3\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t\wt{\bfZ}_{1}} + \norm[F]{\wt{\bfT}_4\t  \overline{\bfB}_{\ell} \wt{\bfZ}_{2}} + \norm[F]{\alpha_{m+1}\wt{\bfT}_3\t \bfE_{m+1,1}\wt{\bfZ}_2}\\
%&\le \sqrt{\ell} \max \{\sigma_{k}, \mathcal{M}_{\a,\b}\} + |\a_{m+1}|,
%\end{align*}
%where $\mathcal{M}_{\alpha,\beta} = \underset{1\le i \le \ell}{\max} (|\alpha_{m+i}| + |\beta_{m+i+1}|)$. So
%\begin{equation}
%\label{eqfrob1}
%\norm[F]{\bfT^{\top}_{c}\bfB_{m+\ell}\bfZ} \le \sigma_{k} + \sqrt{\ell}\max{\{\sigma_{k}, \mathcal{M}_{\alpha,\beta}\}} + |\alpha_{m+1}|.
%\end{equation}
%where $\mathcal{C}_{m,k,\ell} = \underset{1\le i \le 3}{\max}{\{\mathcal{C}^{i}_{m,k,\ell}\}}$.
%\begin{align}
%\bfT^{\top}\bfB_{m+\ell}\bfZ_{c} &= \begin{bmatrix}{\bf\Psi}_{k-1}\t & \bfO_{(k-1) \times \ell} \\ \eta\t & \bfO_{1 \times \ell} \\ \wt{\bfT}_{1}\t & \wt{\bfT}_{2}\t \end{bmatrix}\begin{bmatrix}\bfB_{m} & \begin{bmatrix}\bfO_{m\times \ell} \\ \alpha_{m+1}\bfe_1\t \end{bmatrix} \\\\ \bfO_{\ell \times m} &  \overline{\bfB}_{\ell}\end{bmatrix}\begin{bmatrix}\wt{\bfZ}_{3} \\ \wt{\bfZ}_{4}\end{bmatrix}\\
%\label{eq:def2}
%&=\begin{bmatrix}{\bf\Psi}_{k-1}\t \bfB_{m}\wt{\bfZ}_{3} + \alpha_{m+1}{\bf\Psi}_{k-1}\t\bfE_{m+1,1}\wt{\bfZ}_{4} \\\\ \eta\t\bfB_{m}\wt{\bfZ}_{3} + \alpha_{m+1}\eta\t\bfE_{m+1,1}\wt{\bfZ}_{4} \\\\
%\wt{\bfT}_{1}\t\bfB_{m}\wt{\bfZ}_{3} + \wt{\bfT}_{2}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4} + \alpha_{m+1}\wt{\bfT}_{1}\t\bfE_{m+1,1}\wt{\bfZ}_{4}\end{bmatrix}
%\end{align}
According to (\ref{SVD}), (\ref{relationship1})-(\ref{relationship3}) and (\ref{eq:perp2}),
\begin{align}
\bfB_{m}\wt{\bfZ}_{3} &= {\bf\Psi}_{m+1}{\bf\Sigma}_{m}{\bf\bfPhi}_{m}\t \wt{\bfZ}_{3}\\
&= \begin{bmatrix}{\bf\Psi}_{k-1}& {\bf\Psi}_{c}\end{bmatrix}\begin{bmatrix}{\bf\Sigma}_{k-1} & \\ & {\bf\Sigma}_{c}\end{bmatrix}\begin{bmatrix}{\bf\Phi}_{k-1}\t \\\\ {\bf\Phi}_{c}\t\end{bmatrix}\wt{\bfZ}_{3}\\
\label{eq:bz}
&= {\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3}.
\end{align}
Since ${\bf\Phi}_c$ is orthogonal complement of ${\bf\Phi}_{k-1}$ and $\wt{\bfZ}_3 \perp {\bf\Phi}_{k-1}$, $\wt{\bfZ}_3 \subset \mathcal{R}({\bf\Phi}_{c})$. Let $\wt{\bfZ}_3 = {\bf\Phi}_{c}{\bf\Theta}$, where coefficient matrix ${\bf\Theta} \in \mathbb{R}^{(m+1-k) \times (m-k)}$. By (\ref{eq:bz}),
\begin{align}
\label{ineq:bz}
\norm[F]{{\bfB}_m\wt{\bfZ}_3}  &= \norm[F]{{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t{\bf\bfPhi}_{c}{\bf\Theta}}\\
&=\norm[F]{{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Theta}}\\
&=\sqrt{\text{trace}({\bf\Theta}\t{\bf\Sigma}_{c}\t{\bf\Psi}_{c}\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Theta})}\\
&=\sqrt{\text{trace}({\bf\Theta}\t{\bf\Sigma}_{c}\t{\bf\Sigma}_{c}{\bf\Theta})}\\
& \le \sqrt{\sigma^2_k\text{trace}({\bf\Theta}\t{\bf\Theta})}\\
&=\sigma_k\sqrt{\text{trace}({\bf\Theta}\t{\bf\bfPhi}_{c}\t{\bf\bfPhi}_{c}{\bf\Theta})}\\
& = \sigma_k\sqrt{\text{trace}(\wt{\bfZ}_3\t\wt{\bfZ}_3)}\\
& = \sigma_k \norm[F]{\wt{\bfZ}_3}.
\end{align}
Since the last row of $\begin{bmatrix}\wt{\bfZ}_2 & \wt{\bfZ}_4 \end{bmatrix}$ is orthonormal,
\begin{align}
\label{ineq:alphaE}
\norm[F]{\alpha_{m+1}\bfE_{m+1,1}\wt{\bfZ}_4} \le |\alpha_{m+1}|.
\end{align}
Based on (\ref{diffright}) and (\ref{ineq_1}),
\begin{align}
\label{totalineq}
\norm[F]{\bfB_{m+\ell}} - \norm[F]{\widehat{\bfB}_{k,\ell}} &\le \sigma_k \norm[F]{\wt{\bfZ}_3} + |\alpha_{m+1}| + \norm[F]{\overline{\mxB}_{\ell}}\norm[F]{\wt{\bfZ}_4}\\
& \le \max\{\sigma_k, \norm[F]{\overline{\mxB}_{\ell}}\}(m-k) + |\alpha_{m+1}|
\end{align}

%Then
%\begin{align*}
%{\bf\Psi}_{k-1}\t\bfB_{m}\wt{\bfZ}_{3} &= {\bf\Psi}_{k-1}\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3}\\
%&= \bfO_{(k-1)\times(m-k)}.
%\end{align*}
%Plug (\ref{eq:bz}) in (\ref{eq:def2}) and then
%\begin{equation*}
%\bfT^{\top}\bfB_{m+\ell}\bfZ_{c} = \begin{bmatrix} \alpha_{m+1}{\bf\Psi}_{k}\t\bfE_{m+1,1}\wt{\bfZ}_{4} \\\\ \eta\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3} + \alpha_{m+1}\eta\t\bfE_{m+1,1}\wt{\bfZ}_{4} \\\\
%\wt{\bfT}_{1}\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3} + \wt{\bfT}_{2}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4} + \alpha_{m+1}\wt{\bfT}_{1}\t\bfE_{m+1,1}\wt{\bfZ}_{4}\end{bmatrix}.
%\end{equation*}
%Since $\bfZ_{c}$, $\begin{bmatrix}\wt{\bfT}^{\top}_{1} \\ \wt{\bfT}_{2}\t\end{bmatrix}$ and $\eta$ have orthonormal column(s),
%\begin{align*}
%\norm[F]{\wt{\bfZ}^{Z}_3}^2 + \norm[F]{\wt{\bfZ}^{Z}_4}^2 &= \norm[F]{\bfZ_{c}}^2 = m-k, \\
%\norm[F]{\wt{\bfT}_{1}}^2 + \norm[F]{\wt{\bfT}_{2}}^2 &= \norm[F]{\begin{bmatrix}\wt{\bfT}_{1}\\ \wt{\bfT}_{2}\end{bmatrix}}^2 = \ell, \\
%\norm[F]{\eta} = 1,
%\end{align*}
%and
%\begin{align*}
%\norm[F]{\alpha_{m+1}{\bf\Psi}_{k}\t\bfE_{m+1,1}\wt{\bfZ}_{4}} &\le |\alpha_{m+1}|, \\
%\norm[F]{\eta\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3} + \alpha_{m+1}\eta\t\bfE_{m+1,1}\wt{\bfZ}_{4}} &\le \norm[F]{\eta\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3}} + \norm[F]{\alpha_{m+1}\eta\t\bfE_{m+1,1}\wt{\bfZ}_{4}}\\ &\le \sigma_{k} + |\alpha_{m+1}|.
%%\norm[F]{\bfU_{Bc}}\norm[F]{\bfV^{T}_{Bc}}\norm[F]{\wt{\bfZ}_{3}}\\
%%&\le \mathcal{D}^{1}_{m,k,\ell}\sigma_{k}.
%\end{align*}
%Similarly,
%\begin{align*}
%\norm[F]{\wt{\bfT}_{1}\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3} + \wt{\bfT}_{2}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4} + \alpha_{m+1}\wt{\bfT}_{1}\t\bfE_{m+1,1}\wt{\bfZ}_{4}} &\le \norm[F]{\wt{\bfT}_{1}\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\bfPhi}_{c}\t\wt{\bfZ}_{3}} + \norm[F]{\wt{\bfT}_{2}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4}} + \norm[F]{\alpha_{m+1}\wt{\bfT}_{1}\t\bfE_{m+1,1}\wt{\bfZ}_{4}}\\
%&\le \sqrt{\ell}\max{\{\sigma_{k}, \mathcal{M}_{\alpha, \beta} \}} + |\alpha_{m+1}|.
%\end{align*}
%Thus,
%\begin{equation}
%\label{eqfrob2}
%\norm[F]{\bfT^{\top}\bfB_{m+\ell}\bfZ_{c}}\le \sigma_{k} + \sqrt{\ell}\max{\{\sigma_{k}, \mathcal{M}_{\alpha, \beta} \}} + 3|\alpha_{m+1}|.
%\end{equation}
%%where $\mathcal{D}_{m,k,\ell} = \underset{1\le i \le 3}{\max}{\{\mathcal{D}^{i}_{m,k,\ell}\}}$.
%\begin{align}
%\bfT_{c}\t\bfB_{m+\ell}\bfZ_{c} &= \begin{bmatrix}\wt{\bfT}_{3}\t & \wt{\bfT}_{4}\t\end{bmatrix}\begin{bmatrix}\bfB_{m} & \begin{bmatrix}\bfO_{m\times \ell} \\ \alpha_{m+1}\bfe_1\t \end{bmatrix} \\\\ \bfO_{\ell \times m} &  \overline{\bfB}_{\ell}\end{bmatrix}\begin{bmatrix}\wt{\bfZ}_{3} \\ \wt{\bfZ}_{4}\end{bmatrix}\\
%\label{eq:def3}
%&= \wt{\bfT}_{3}\t\bfB_{m}\wt{\bfZ}_{3} + \wt{\bfT}_{4}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4} + \alpha_{m+1}\wt{\bfT}_{3}\t \bfE_{m+1,1}\wt{\bfZ}_{4}.
%\end{align}
%Based on (\ref{eq:perp1}) and (\ref{eq:perp2}),
%\begin{align*}
%\wt{\bfT}_{3}\t\bfB_{m}\wt{\bfZ}_{3} &= \wt{\bfT}_{3}\t\begin{bmatrix}{\bf\Psi}_{k} & {\bf\Psi}_{c}\end{bmatrix}\begin{bmatrix}{\bf\Sigma}_{k-1} & \\ & {\bf\Sigma}_{c}\end{bmatrix}\begin{bmatrix}{\bf\Phi}_{k-1}\t \\\\ {\bf\Phi}_{c}\t\end{bmatrix}\wt{\bfZ}_{3}\\
%&= \wt{\bfT}_{3}\t{\bf\Psi}_{c}{\bf\Sigma}_{c}{\bf\Phi}_{c}\t\wt{\bfZ}_{3}.
%\end{align*}
%Then
%\begin{align*}
%\norm[F]{\wt{\bfT}_{3}\t\bfB_{m}\wt{\bfZ}_{3} + \wt{\bfT}_{4}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4}} &\le \sqrt{\ell}\max \{\sigma_{k}, \mathcal{M}_{\alpha,\beta}\}.
%\norm[F]{\wt{\bfT}^{T}_{3}}\norm[F]{\bfU_{Bc}}\norm[F]{\bfV^{T}_{Bc}}\norm[F]{\wt{\bfZ}_{3}}\\
%&\le \mathcal{E}^{1}_{m,k,\ell}\sigma_{k},
%\end{align*}
%and
%\begin{align*}
%\norm[F]{\wt{\bfT}_{4}\t \overline{\bfB}_{\ell}\wt{\bfZ}_{4}} &\le \norm[F]{\wt{\bfT}^{T}_{4}} \norm[F]{ \overline{\bfB}_{\ell}}\norm[F]{\wt{\bfZ}_{4}}\\
%&\le \mathcal{E}^{2}_{m,k,\ell}\mathcal{M}_{\alpha,\beta}.
%\end{align*}
%By (\ref{eq:def3}),
%\begin{align}
%\label{eqfrob3}
%\norm[F]{\bfT_{c}^{\top}\bfB_{m+\ell}\bfZ_{c}} &\le \sqrt{\ell}\max \{\sigma_{k}, \mathcal{M}_{\alpha,\beta}\} + |\alpha_{m+1}|
%%\norm[F]{\wt{\bfT}^{T}_{3}\bfB_{m}\wt{\bfZ}_{3}} + \norm[F]{\wt{\bfT}^{T}_{4} \overline{\bfB}_{\ell}\wt{\bfZ}_{4}}\\
%%&\le \mathcal{E}^{1}_{m,k,\ell}\sigma_{k} + \mathcal{E}^{2}_{m,k,\ell}\mathcal{M}_{\alpha,\beta}\\
%%\label{eqfrob3}
%%&\le \mathcal{E}_{m,k,\ell}\max{\{\sigma_{k}, \mathcal{M}_{\alpha,\beta} \}},
%\end{align}
%where $\mathcal{E}_{m,k,\ell} = \max{\{\mathcal{E}^{1}_{m,k,\ell}, \mathcal{E}^{2}_{m,k,\ell} \}}$.
%According to (\ref{eq:bbhat}) and the definition of $\mathcal{M}_{\alpha,\beta}$,
%\begin{equation}
%\label{eq:frobupbd}
%\norm[F]{\bfB_{m+\ell}} - \norm[F]{\widehat{\bfB}_{k,\ell}} \le 3\sqrt{\ell}\underset{1\le i \le \ell}{\max}{\{\sigma_{k},(|\alpha_{m+i}| + |\beta_{m+i+1}|)\}} + 2\sigma_{k} + 5|\alpha_{m+1}|.
%\end{equation}
%where $C_{m,k,\ell} = \max{\{\mathcal{C}_{m,k,\ell}, \mathcal{D}_{m,k,\ell}, \mathcal{E}_{m,k,\ell} \}}$.
\end{proof}
\end{theorem}


==> macro_list.tex <==
% general header (fold)
\RequirePackage{amsfonts}
\RequirePackage{amsmath}
\RequirePackage{mathtools}
\RequirePackage{alltt, moreverb}
\RequirePackage{showkeys, showidx}
\RequirePackage{graphicx}
\RequirePackage[utf8]{inputenc}
% \usepackage{algorithm,algpseudocode}
% \renewcommand{\algorithmiccomment}[1]{{(\sf #1)}}
\RequirePackage{color, colortbl}
\RequirePackage{rotating}
\RequirePackage{boxedminipage}
\RequirePackage{upgreek}
\RequirePackage{subfigure}
\usepackage{textcomp}
\usepackage{multirow}
\usepackage{caption}
\usepackage{mathabx}
% \captionsetup[algorithm]{format=hang,singlelinecheck=false}
% special header (fold)
% \newcommand{\widebar}{\bar}
% \newcommand{\widecheck}{\check}
\def\wh{\widehat}
\def\wt{\widetilde}


\newcommand{\fro} {\rm F}                                  % define Frobenius norm
\newcommand{\eps} {\varepsilon}                            % redefine epsilon
\newcommand{\D}   {{\rm D}}                                % differential D
\newcommand{\tol} {{\rm tol}}                              % tolerance
\newcommand{\e}   {\textnormal{e}}                         % Eulerian number
\newcommand{\clos}{\textnormal{Closure}}                   % closure
\newcommand{\im}  {\textnormal{Im }}                       % imaginary part
\newcommand{\re}  {\textnormal{Re }}                       % real part
\newcommand{\hf}  {\frac{1}{2}}                            % 1/2
\DeclareMathOperator*{\argmin}{arg\,min}                   % arg min
\DeclareMathOperator*{\argmax}{arg\,max}                   % arg max
\renewcommand{\i} {\textnormal{i}}                         % imaginary unity
\renewcommand{\t} {^{\top}}                                % transpose, e.g. $A\t$
\renewcommand{\d} {{\rm d}}                                % differential d
\renewcommand{\H} {^{{\rm H}}}                             % Hermitian
\newcommand{\norm} [2][]{\left\|#2\right\|_{#1}}           % f.e. \norm[\infty]{A-B}
\newcommand{\abs}  [2][]{\left|#2\right|_{#1}}             % f.e. \abs[\infty]{A-B}
\newcommand{\cond} [2][]{{\rm cond}_{#1}\left( #2 \right)} % f.e. \cond[\infty]{A}
\newcommand{\pow}  [1]  {^{\left(#1\right)}}               % brackets exponent
\newcommand{\sign} [1]  {{\rm sign\!}\left( #1 \right)}    % signum
\newcommand{\spann}[1]  {{\rm span\!}\left( #1 \right)}    % span of a function
\newcommand{\ran}[1]{\mathrm{range}(#1)}                  % rangefM of a matrix
% \renewcommand{\diag} [1]  {{\rm diag\!}\left( #1 \right)}    % diagonal of a matrix
\renewcommand{\ker}[1]  {{\rm ker\!}\left( #1 \right)}     % kernel of a function
\renewcommand{\vec}[1]  {{\rm vec}\left( #1 \right)}     % kernel of a function
% \renewcommand{\rank}[1]  {{\rm rank}\left( #1 \right)}     % kernel of a function
\newcommand{\ul}   [1]  {\underline{#1}}                   % shorted underline
\newcommand{\trace}{\mathsf{trace}}
% \newcommand{\email}[1]  {\texttt{#1}}                      % email
\newcommand{\kron}{\otimes}                                % kronecker product
\newcommand{\acknowledgement}[1]{\noindent\textbf{Acknowledgement: }#1}   % acknowledgement

\newcommand{\bmx}{\left[ \begin{array}}
\newcommand{\emx}{\end{array} \right]}

% -------------
% equations
\newcommand{\eqs}{\begin{eqnarray}}
\newcommand{\eqe}{\end{eqnarray}}
\newcommand{\eqsn}{\begin{eqnarray*}}
\newcommand{\eqen}{\end{eqnarray*}}

% -----------------------------
% <<< regular Greek >>>
\def\a{\alpha}
\def\b{\beta}
\def\c{\gamma}
\def\C{\Gamma}
\def\d{\delta}
\def\D{\Delta}
\def\e{\varepsilon}
\def\es{\epsilon}
\def\z{\zeta}
\def\h{\eta}
\def\H{\Eta}
\def\v{\vartheta}
\def\vs{\theta}
\def\VC{\Theta}
\def\i{\iota}
\def\k{\kappa}
\def\l{\lambda}
\def\L{\Lambda}
\def\m{\mu}
\def\n{\nu}
\def\q{\xi}
\def\Q{\Xi}
\def\p{\pi}
\def\P{\Pi}
\def\r{\rho}
\def\s{\sigma}
\def\Si{\Sigma} % for SIAM Jrns \S is section symbol
% \def\t{\tau}
\def\f{\varphi}
\def\fs{\phi}
\def\F{\Phi}
\def\x{\chi}
\def\X{{\cal X}}
\def\y{\psi}
\def\Y{\Psi}
\def\o{\omega}
\def\O{\Omega}



% ---------------------------------------------------------------------------
% bold greek and latin characters and bold numbers (requires amsmath) (fold)

\newcommand{\bfGamma}{{\boldsymbol{\Gamma}}}
\newcommand{\bfDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bfTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bfLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\bfXi}{{\boldsymbol{\Xi}}}
\newcommand{\bfPi}{{\boldsymbol{\Pi}}}
\newcommand{\bfSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bfUpsilon}{{\boldsymbol{\Upsilon}}}
\newcommand{\bfPhi}{{\boldsymbol{\Phi}}}
\newcommand{\bfPsi}{{\boldsymbol{\Psi}}}
\newcommand{\bfOmega}{{\boldsymbol{\Omega}}}
\newcommand{\bfalpha}{{\boldsymbol{\alpha}}}
\newcommand{\bfbeta}{{\boldsymbol{\beta}}}
\newcommand{\bfgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bfdelta}{{\boldsymbol{\delta}}}
\newcommand{\bfepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bfvarepsilon}{{\boldsymbol{\varepsilon}}}
\newcommand{\bfzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\bftheta}{{\boldsymbol{\theta}}}
\newcommand{\bfvartheta}{{\boldsymbol{\theta}}}
\newcommand{\bfiota}{{\boldsymbol{\iota}}}
\newcommand{\bfkappa}{{\boldsymbol{\kappa}}}
\newcommand{\bflambda}{{\boldsymbol{\lambda}}}
\newcommand{\bfmu}{{\boldsymbol{\mu}}}
\newcommand{\bfnu}{{\boldsymbol{\nu}}}
\newcommand{\bfxi}{{\boldsymbol{\xi}}}
\newcommand{\bfo}{{\boldsymbol{o}}}
\newcommand{\bfpi}{{\boldsymbol{\pi}}}
\newcommand{\bfvarpi}{{\boldsymbol{\varpi}}}
\newcommand{\bfrho}{{\boldsymbol{\rho}}}
\newcommand{\bfvarrho}{{\boldsymbol{\varrho}}}
\newcommand{\bfsigma}{{\boldsymbol{\sigma}}}
\newcommand{\bfvarsigma}{{\boldsymbol{\varsigma}}}
\newcommand{\bftau}{{\boldsymbol{\tau}}}
\newcommand{\bfupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\bfphi}{{\boldsymbol{\phi}}}
\newcommand{\bfvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\bfchi}{{\boldsymbol{\chi}}}
\newcommand{\bfpsi}{{\boldsymbol{\psi}}}
\newcommand{\bfomega}{{\boldsymbol{\omega}}}
\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfO}{{\bf O}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfzero}{{\bf0}}
\newcommand{\bfone}{{\bf1}}
\newcommand{\bftwo}{{\bf2}}
\newcommand{\bfthree}{{\bf3}}
\newcommand{\bffour}{{\bf4}}
\newcommand{\bffive}{{\bf5}}
\newcommand{\bfsix}{{\bf6}}
\newcommand{\bfseven}{{\bf7}}
\newcommand{\bfeight}{{\bf8}}
\newcommand{\bfnine}{{\bf9}}


\newcommand{\mxA}{{\bf A}}
\newcommand{\mxB}{{\bf B}}
\newcommand{\mxC}{{\bf C}}
\newcommand{\mxD}{{\bf D}}
\newcommand{\mxE}{{\bf E}}
\newcommand{\mxF}{{\bf F}}
\newcommand{\mxG}{{\bf G}}
\newcommand{\mxH}{{\bf H}}
\newcommand{\mxI}{{\bf I}}
\newcommand{\mxJ}{{\bf J}}
\newcommand{\mxK}{{\bf K}}
\newcommand{\mxL}{{\bf L}}
\newcommand{\mxM}{{\bf M}}
\newcommand{\mxN}{{\bf N}}
\newcommand{\mxO}{{\bf O}}
\newcommand{\mxP}{{\bf P}}
\newcommand{\mxQ}{{\bf Q}}
\newcommand{\mxR}{{\bf R}}
\newcommand{\mxS}{{\bf S}}
\newcommand{\mxT}{{\bf T}}
\newcommand{\mxU}{{\bf U}}
\newcommand{\mxV}{{\bf V}}
\newcommand{\mxW}{{\bf W}}
\newcommand{\mxX}{{\bf X}}
\newcommand{\mxY}{{\bf Y}}
\newcommand{\mxZ}{{\bf Z}}
\newcommand{\mxSigma}{{\bf \Sigma}}

% (end)

% ---------------------------------------------------------------------------
% caligraphic characters (fold)

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
% (end)

% ---------------------------------------------------------------------------
% blackboard characters (requires amsfont) (fold)

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

\newcommand{\sfE}{{\sf E}}


\newcommand{\true}{\mathrm{true}}
\newcommand{\filter}{\mathrm{filter}}
\newcommand{\tsvd}{\mathrm{tsvd}}
\newcommand{\tik}{\mathrm{tik}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\spl}{\mathrm{spl}}
\newcommand{\wie}{\mathrm{Wiener}}
\newcommand{\smooth}{\mathrm{smooth}}
\newcommand{\con}{\mathrm{con}}
\newcommand{\ssvd}{\mathrm{ssvd}}
\newcommand{\inv}{\mathrm{inv}}
\newcommand{\mse}{\mathrm{MSE}}
\newcommand{\ERR}{\mathrm{ERR}}

% \newcommand{\eqdef}{\overset{{\rm def}}{=}}
\def\Tiny{\fontsize{4pt}{4pt}\selectfont}
\newcommand*{\eqdef}{\ensuremath{\overset{\mathclap{\text{\Tiny def}}}{=}}}

% empty line
\def\el{\vspace{11pt}\noindent} % better actual 1 vertical line

% short hand for symbols
\def\eqv{\Leftrightarrow}
\def\imp{\Rightarrow}

% matrices
\newcommand{\ars}[1]{\left[ \begin{array}{#1}}
\newcommand{\are}{\end{array} \right] }
\newcommand{\oars}[1]{\begin{array}{#1}}
\newcommand{\oare}{\end{array}}
\newcommand{\rars}[1]{\left( \begin{array}{#1}}
\newcommand{\rare}{\end{array} \right) }

\newtheorem{conj}{Conjecture}
%\begin{thm}[Main Theorem]
%This is the main theorem.
%\end{thm}

